Active Perception and Control from Temporal Logic Specifications

Next-generation autonomous systems must execute complex tasks in uncertain environments. Active perception, where an autonomous agent selects actions to increase knowledge about the environment, has gained traction in recent years for motion planning under uncertainty. One prominent approach is planning in the belief space. However, most belief-space planning starts with a known reward function, which can be difficult to specify for complex tasks. On the other hand, symbolic control methods automatically synthesize controllers to achieve logical specifications, but often do not deal well with uncertainty. In this work, we propose a framework for scalable task and motion planning in uncertain environments that combines the best of belief-space planning and symbolic control. Specifically, we provide a counterexample-guided-inductive-synthesis algorithm for probabilistic temporal logic over reals (PRTL) specifications in the belief space. Our method automatically generates actions that improve confidence in a belief when necessary, thus using active perception to satisfy PRTL specifications.

==> 1_intro2.tex <==


\textit{Taskable} and \textit{adaptive} \gls*{ips}  must not only plan and execute actions to satisfy high-level, possibly vague, task specifications but also be able to change their behaviors over time, learning from their own experiences and those of other entities, such as other \gls*{ips} or humans, and from instruction or observation. These systems must perceive the world and extrapolate beliefs about the future behavior of the environment, explicitly acting to improve confidence in this belief. This behavior is an active learning process and does not passively receive information from a teacher; the system explicitly interacts with the environment to gather more information to improve its knowledge. Over the years, the topic of perception has been studied by philosophers and scientists alike. However, the concept of active perception in engineering was introduced more recently when Bajcsy \cite{bajcsy1988active} wrote:

\begin{quote}
``Active sensing is the problem of intelligent control strategies applied to the data acquisition process which will depend on the current state of data interpretation including recognition.''
\end{quote}   

Active perception is not a pure control theory: the feedback is performed not only on sensory data but also in data processing. Thus, the feedback is dependent on a priori knowledge and models of the agent's world. For that, the perception must be modeled such that its intrinsic uncertainties are fed back to control the data acquisition process. It is not pure machine learning as well: the agent actively chooses activities to gain information. For example, when asking a robot to fetch a cup that is on a table for us, we do not want to give the task in the robot's coordinates, but merely state that it is on the table. Then, it is the robot's job to use this imperfect information to make observations, learn the cup coordinates, grasp and deliver the cup to us. Although gathering parameters and errors for the perception model is a challenging problem; it is an essential problem. Accepting incomplete, noisy data as a matter of fact and incorporating it in the control synthesis strategy is of fundamental importance for reliable knowledge construction. 

The design of intelligent systems which can learn and act to construct the necessary knowledge to achieve a goal is a problem of practical importance. Many applications in robotics (e.g., navigation, manipulation, and surgery) and autonomous systems (e.g., unmanned aircraft and self-driving cars) must deal explicitly with uncertainty. Even considering reliable sensing, robots, for example, cannot see, immediately, inside boxes, behind walls, or into nuclear containment vessels. Many ideas and methods for how to handle such uncertainty using active perception have been proposed in the past. However, still, there is no computationally tractable solution in myriad real applications \cite{bajcsy2018revisiting}. Therefore, we address this challenge by developing a collection of novel techniques which combines active learning and \gls*{itmp}.

We propose a novel \gls*{prstl} controller synthesis algorithm for systems with perception and actuation uncertainty based on \gls*{cegis} \cite{alur2013syntax,reynolds2015counterexample}. By separating discrete task planning and continuous motion planning, we find trajectories that robustly satisfy \gls*{prstl} specifications.  

Discrete planning is based on efficient on-the-fly partitioning from \gls*{prstl} predicates, and thus does not require a priori partitioning of the workspace. Satisfying discrete plans are found using an efficient \gls*{csp} solver and sent to the continuous layer, which checks dynamic feasibility via sampling-based motion planning. If a discrete plan is dynamically infeasible, it is sent back to the discrete planner as a counterexample, where it is used to generate a new candidate discrete plan. Once a feasible discrete plan is found, we use a novel formulation of \textit{robust \gls*{prstl} semantics} (which extends \gls*{stl} qualitative semantics) to find a continuous plan that satisfies the specification with maximal robustness. Finally, we track this continuous plan with a robust controller. Our approach is scalable to systems with high-dimensional dynamics and non-convex task specifications. Furthermore, since all reasoning is in the belief space, our approach naturally incorporates active perception in the planning process. 


One popular way to handle the observation uncertainty during the planning is assume the \gls*{mlo} \cite{platt2010belief} and replanning techniques during execution. This approach have been successfuly used in robotics \cite{kaelbling2013integrated,hadfield2015modular} using planning techniques in Artificial Intelligence such as Fast-Forward \cite{hoffmann2001ff}. As shown in \cite{platt2010belief}, a run in the belief space for a Gaussian process can be tracked using a \gls*{lqg} framework or using other control techniques for stochastic systems such that \cite{van2012motion}.     

==> 2_relatedwork.tex <==
\section{Related Work}\label{sec:idprstl_relatedwork}

Active perception can be formalized as a \gls*{pomdp} \cite{krishnamurthy2016partially} since physical systems often follow the Markov assumption. \gls*{pomdp} planning involves a search for a policy that satisfies certain requirements. Since states are not directly observable, the policy is a mapping from history, a sequence of observations and actions, to new actions. History can be compactly represented as a probability distribution over state space called the \textit{belief}, which is a sufficient statistic for history. 

Various methods have been proposed for active perception via belief space planning, most of which search for a policy that maximizes the expected value of a reward function.  Point-based value iteration methods \cite{porta2006point,bai2014integrated} compute a control policy over the belief space by selecting a limited set of representative points and iteratively applying value updates. Simulation-based methods \cite{valencia2013planning} generate and compare several candidate plans, while sampling-based methods \cite{prentice2009belief,hauser2010randomized,bry2011rapidly,hollinger2013stochastic,agha2014firm} search for an optimal plan using randomized strategies. Policy search methods \cite{deisenroth2012solving} use approximate inference in Gaussian belief spaces to directly optimize parameters of a control policy, and trajectory optimization methods \cite{platt2010belief,van2011lqg,van2012efficient,patil2014gaussian,indelman2016towards} compute open loop trajectories in the belief space. All of these methods rely on an a priori specified reward function, the maximization of which leads to desirable behavior. 

Specifying a reward function that guarantees completion of a complex, high-level task can be difficult, however. Using temporal logic specifications is often clearer and more intuitive. Furthermore, \textit{symbolic control} approaches, which synthesize controllers to achieve logical specifications, can provide strong theoretical guarantees. However, existing symbolic control methods either assume a deterministic environment or model uncertainty only as part of the dynamics of the system. In this work, we provide a robust and scalable framework for \textit{symbolic control in the belief space} based \gls*{prstl} \cite{sadigh2015safe} specifications. 
 
Existing \gls*{prstl} controller synthesis methods include mixed integer \gls*{socp} \cite{sadigh2015safe,zhong2017fast}, sampling-based optimization \cite{dey2016fast}, and \gls*{rhc} \cite{yoo2015control}. \gls*{socp} and sampling-based methods provide satisfying controllers for a convex fragment of \gls*{prstl}, but do not incorporate a perception model in the system dynamics. Thus these algorithms cannot synthesize controls to gather more information, and therefore are not considered active perception methods. \gls*{rhc} methods can use active perception, but again are restricted to a convex fragment of \gls*{prstl} and rely on aggressive heuristics at the expense of completeness. 

Unlike other active perception via belief space planning where tasks are described by a reward function \cite{porta2006point,bai2014integrated,valencia2013planning,prentice2009belief,hauser2010randomized,bry2011rapidly,hollinger2013stochastic,agha2014firm,platt2010belief,van2011lqg,van2012efficient,patil2014gaussian,indelman2016towards}, our method guarantee a high-level specification in \gls*{prstl} language. Diferently from previous approach in symbolic control from \gls*{prstl} specifications \cite{sadigh2015safe,zhong2017fast,dey2016fast,yoo2015control}, we model the learning dynamics of Bayesian filters to incoporate not only task and motion planning but also active perception. Furtermore, we do not limit the synthesis for a convex fragment of \gls*{prstl} and a short-time horizon. We react to unexpected observations using feedback controllers and replanning.  
